On the Relevance of Temporal Features for Medical Ultrasound Video Recognition

Many medical ultrasound video recognition tasks involve identifying key anatomical features regardless of when they appear in the video suggesting that modeling such tasks may not benefit from temporal features. Correspondingly, model architectures that exclude temporal features may have better sample efficiency. We propose a novel multi-head attention architecture that incorporates these hypotheses as inductive priors to achieve better sample efficiency on common ultrasound tasks. We compare the performance of our architecture to an efficient 3D CNN video recognition model in two settings: one where we expect not to require temporal features and one where we do. In the former setting, our model outperforms the 3D CNN - especially when we artificially limit the training data. In the latter, the outcome reverses. These results suggest that expressive time-independent models may be more effective than state-of-the-art video recognition models for some common ultrasound tasks in the low-data regime.

==> author.tex <==
\author{D. Hudson Smith\inst{1} \and
John Paul Lineberger\inst{1} \and
Hamilton Baker \inst{2}}
%
\authorrunning{D. Smith et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{Clemson University, Clemson SC 29631, USA
\email{\{dane2,jplineb\}@clemson.edu} \and
MUSC, Charleston SC 29425, USA
\email{baker@musc.edu}}
